The SynCOM Flow Tracking Challenge

Understanding solar wind flows is crucial for unraveling the dynamics of the Sun's corona and improving space weather forecasting. However, the complex nature of the solar wind and the absence of reliable ground-truth data present significant challenges to current tracking methods. To address this, the Flow Tracking Challenge was established, providing a platform for testing and refining flow tracking algorithms using synthetic images generated by the Synthetic Coronal Outflow Model (SynCOM). The challenge is divided into two phases: a preliminary phase focusing on simpler flow scenarios and a main phase featuring more complex synthetic images that mimic solar outflows. These phases allow researchers to evaluate their methods under various simulated conditions. SynCOM's synthetic data benchmark improves accuracy in velocity estimations. This paper presents the preliminary results of the Flow Tracking Challenge, where the synthetic images from SynCOM are used to test solar wind velocity tracking methods. Initial findings demonstrate SynCOM's value as a benchmark, guiding improvements for upcoming missions like PUNCH.

==> draft.tex <==
% The accurate tracking of solar wind flows is essential for understanding the dynamics of the corona and the impact of the solar wind on space weather. Current methods face challenges due to the complex and variable nature of the solar wind, compounded by the lack of ground-truth data for validation. The \textit{Flow Tracking Challenge} was created to address this challenge, providing a platform for the scientific community to evaluate and improve various flow tracking algorithms using SynCOM's synthetic images that mimic coronal outflows \citep{moraes_filho_2024}. This initiative fosters collaboration and innovation, helping researchers refine their methods and enhance future solar wind tracking, particularly for observational missions like PUNCH.

% The PUNCH (Polarimeter to Unify the Corona and Heliosphere) mission, launching in 2025, aims to deliver high-resolution, 3D polarized observations of solar wind structures transitioning from the corona into the inner heliosphere \citep{DeForest_2022}. As part of NASA's Small Explorer program, PUNCH consists of three Wide Field Imagers (WFIs) covering 20 to 180 solar radii, and one Narrow Field Imager (NFI) focused on 6 to 32 solar radii. These instruments will capture both small-scale features and global structures, with polarization playing a key role in deducing the 3D structure of the solar wind and understanding the evolution of CMEs and other transients \citep{deforest_2016}. By mapping both large-scale dynamics and transient features, PUNCH will enhance the SynCOM model, providing crucial data on solar wind acceleration and turbulence, ultimately improving our understanding of the solar wind transition from the corona to the heliosphere.

% This paper is structured as follows: Section \ref{s-motivation_FT} covers the motivation behind the Flow Tracking Challenge and the need for accurate solar wind velocity measurements. Section \ref{S-methodology_FT} details the methodology, focusing on the exercises used to test the tracking algorithms. Section \ref{S-challenge-FT} discusses the specific challenges and limitations of current tracking methods. Finally, Section \ref{S-reults-FT} presents the results of the challenge, emphasizing SynCOM's role in validating tracking methods.

%%%%%%%%%


% This paper presents the SynCOM flow tracking challenge hosted by Catholic University, which provides SynCOM-generated synthetic images for researchers to use to validate their models. By comparing their algorithms with known ground truth, researchers can refine their methods and improve the accuracy of flow tracking for future missions such as PUNCH.


%%%%%%%%%





% \section{Introduction}
%      \label{S-Introduction} 

% This file describes the use of special \LaTeX\ features,
% useful to format an article for {\it Solar Physics}.  It is only a complement
% to the \LaTeX\ and \BibTeX\ documentation.  
% It is designed to be used as an example
% article giving the general commands. When compiled with \LaTeX\ 
% (see Sect.~\ref{S-BibTeX} for \BibTeX\ compilation), it provides
% some practical guidance on the main useful features. More information
% is included within this file, but commented out (with a \%).
% Un-commenting the \LaTeX\ commands permits one to show their 
% results in the compiled file.   
    
%   %{\bf --- Road map of the article} \\
%     % When writing a article, it is worth to define a title for each paragraph:
%     %   gives a roadmap for the article logic.
%     % Replacing automatically all the ``%{\bf'' by ``{\bf'' 
%     % brings these titles in the typeset of the article.
%  Section~\ref{S-general} gives examples and some general information
% to aid writing text with citations (Sect.~\ref{S-text})
% and defining labels (Sect.~\ref{S-labels}).
% Section~\ref{S-features} gives examples of equations 
% (Sect.~\ref{S-equations}), figures (Sect.~\ref{S-figures}), and 
% tables (Sect.~\ref{S-tables}).
% It continues by describing the inclusion of labeled references
% (Sect.~\ref{S-references}) and suggestions for an easy construction 
% of a list of references (Sect.~\ref{S-BibTeX}). 
% An appendix is shown as a particular section (Appendix~\ref{S-appendix}),
% which can contain figures and tables (Fig.~\ref{F-appendix}, 
% Table~\ref{T-appendix}).
% There is a list of abbreviations used for the main journals (see the
% beginning of this \texttt{.tex} file for the definition of the \LaTeX\ commands.
% Our conclusions are given in Sect.~\ref{S-Conclusion}. 


% \section{Motivation}
% \label{S-aug}

% The increasing necessity to evaluate the performance of existing flow tracking algorithms over a broad range of heliocentric distances, unrestricted by the field of view of prior coronagraphs, is acknowledged. To fulfill this requirement, we are developing a collection of data-driven numerical models of a dynamic solar corona, based on previous observations. These models reproduce a transient, quasi-periodic plasma outflow that simulates the real solar corona's behavior. Given that the models come with predefined flow parameters, they can serve as a benchmark for assessing various data analysis methods aimed at measuring radial velocity and acceleration in the corona. This allows for comparison of accuracy and performance among different flow-tracking codes.

% Validating flow tracking algorithms using synthetic flow models such as the ones collected on this page can be instrumental for current and upcoming coronal imaging missions, such as the Polarimeter to Unify the Corona and Heliosphere (PUNCH) mission \citep{DeForest_2022}.

% The models are grouped into two categories: 1-dimensional time-evolving models based on synthetic distance-time (DT) plots (Preliminary Challenge) and more sophisticated 2-dimensional time-evolving models generated by the SynCOM code described below (Main Challenge). In either case, the task is to measure the parameters listed below.
 
% \section{The Challenge} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       \label{S-general}      

% TARGET VARIABLES
% Identify the following flow metrics for each model:
% 1) mean radial velocity [km / s] 2) velocity standard deviation [km / s] 3) mean radial acceleration [$km/s^2$] 4) acceleration standard deviation [$km/s^2$] 5) mean period of disturbances [s]
% Symbols: $dt$, image frequency; $dr$, radial pixel resolution; $d\theta$, angular position resolution per pixel. Data sets come in two formats: FITS or IDL SAVE. SynCOM-based models provide extra features.



% \subsection{Preliminary Challenge} %%%%%%%%%%%%%%
%   \label{S-text}
% The current section contains synthetic DT plots stored as 2 dimensional FITS and SAV data arrays. Below is an example explaining the coordinate system used. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.7\linewidth]{Figures/dt-plot_preliminary challenge.png}
%     \caption{Synthetic distance-time plots. These image represents a snapshot of the flow at a given position angle.}
%     \label{fig:dt-plot_preliminary}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/model_00.png}
%     \caption{Preliminary sample challenge. This distance-time graph was produced using a propagation velocity of $75$ km/s with a periodic interval of $1200$ seconds. The temporal and spatial resolution for this example are 24 seconds and 435 kilometers, respectively.}
%     \label{fig:example_model}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\linewidth]{Figures/model_01.png}
%     \includegraphics[width=0.45\linewidth]{Figures/model_02.png} \\
%     \includegraphics[width=0.45\linewidth]{Figures/model_03.png}
%     \includegraphics[width=0.45\linewidth]{Figures/model_04.png} \\
%     \includegraphics[width=0.45\linewidth]{Figures/model_05.png}
%     \includegraphics[width=0.45\linewidth]{Figures/model_06.png}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}
    
% \begin{itemize}

%     \item dt = 12s, dr = 435 km
    
%     \item dt = 12s, dr = 435 km

%     \item dt = 300s, dr = 9744 km

%     \item dt = 300s, dr = 9744 km

%     \item dt = 300s, dr = 9744 km

%     \item dt = 300s, dr = 9744 km
% \end{itemize}

% \subsection{Main Challenge} %%%%%%%%%%%%%%
%   \label{S-labels}

% To enhance the precision of coronal flow models, we are developing SynCOM (Synthetic Corona Outflow Model) code, an empirical data-driven framework for a dynamic solar corona based on previous high-resolution observations. SynCOM replicates the transient and quasi-periodic behavior observed in the actual solar corona. The generated synthetic images display a realistic radial scaling of polarized brightness and incorporate stochastic elements to account for physical plasma outflow fluctuations and instrumental noise. The model employs a predefined probability distribution of flow velocity and features an adjustable signal-to-noise ratio, which can be used to evaluate the accuracy of flow velocity algorithms under various observational conditions. It may also encompass radial flow acceleration and other realistic coronal outflow characteristics. 
%  \begin{figure}
%      \centering
%      \includegraphics[width=0.7\linewidth]{Figures/syncom_coordinates.png}
%      \caption{Caption}
%      \label{fig:enter-label}
%  \end{figure}
% The SynCOM models presented below are encapsulated in 3D data arrays (FITS and IDL SAVE formats) and also include video files showcasing the simulated plasma flow. The 3D arrays consist of time-sequenced individual image frames, which can be used to produce DT plots as shown below and can be analyzed directly.


   
% \section{Conclusion} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \label{S-Conclusion} 
%       We hope authors of {\it Solar Physics} will find this guide useful.
% Please send us feedback on how to improve it.
      
%   \LaTeX\ is very convenient to write a scientific text, in particular
% with the use of labels for figures, tables, and references. Moreover, the labels and list of references are checked by the software against
% one another, and, the formatting should be effortless with \BibTeX.



%%%%%%%%
